Real Space Invariants: Twisted Bulk-Boundary Correspondence of Fragile Topology

In this paper, we propose a new type of bulk-boundary correspondence as a generic approach to theoretically and experimentally detect fragile topological states. When the fragile phase can be written as a difference of a trivial atomic insulator and the so-called obstructed atomic insulator, the gap between the fragile phase and other bands must close under a specific novel twist of the boundary condition of the system. We explicitly work out all the twisted boundary conditions (TBC) that can detect all the 2D fragile phases implied by symmetry eigenvalues in all wallpaper groups. We develop the concept of real space invariants - local good quantum numbers in real space - which fully characterize the eigenvalue fragile phases. We show that the number of unavoidable level crossings under the twisted boundary condition is completely determined by the real space invariants. Possible realizations of the TBC of the fragile band in metamaterial systems are discussed.

==> table_PGI_PBC.tex <==
\begin{tabular}{|c|L{4cm}|L{4cm}|L{4cm}|L{4cm}|}
\hline
 & NSOC, NTRS & NSOC, TRS & SOC, NTRS & SOC, TRS\\
\hline
\hline
\multirow{1}{*}{$2$}& $\delta_{1}^{\rm G} = 4\delta_1$ & $\delta_{1}^{\rm G} = 4\delta_1$ & $\delta_{1}^{\rm G} = 4\delta_1$ & $\delta_{1}^{\rm G} = 0\mod2$\\
\hline
\multirow{1}{*}{$m^\pr$}& $\delta_{1}^{\rm G} = 2\delta_1$ & $\delta_{1}^{\rm G} = 2\delta_1$ & $\delta_{1}^{\rm G} = 2\delta_1$ & $\delta_{1}^{\rm G} = 0\mod2$\\
\hline
\multirow{1}{*}{$m^\prpr$} & $\delta_{1}^{\rm G} = \delta_1$ & $\delta_{1}^{\rm G} = \delta_1$ & $\delta_{1}^{\rm G} = \delta_1$ & $\delta_{1}^{\rm G} = \delta_1\mod2$\\
\hline
\multirow{1}{*}{$2mm$}& $\delta_{1}^{\rm G} = 4\delta_1$ & $\delta_{1}^{\rm G} = 4\delta_1$ & & $\delta_{1}^{\rm G} = 0\mod2$ \\
\hline
\multirow{3}{*}{$4$}& $\delta_{1}^{\rm G} = 3\delta_1 + \delta_3 -\delta_2$ & $ \delta_{1}^{\rm G} = 4\delta_1 - \delta_2$ &  $\delta_{1}^{\rm G} = 3\delta_1 + \delta_3 -\delta_2$ & $\delta_{1}^{\rm G} = 2\delta_1$\\
& $\delta_{2}^{\rm G} = 2\delta_2$ & $ \delta_{2}^{\rm G} =2\delta_2$ & $\delta_{2}^{\rm G} = 2\delta_2$ & $\delta_{2}^{\rm G} = 0\mod2$\\
& $\delta_{3}^{\rm G} = 3\delta_3+\delta_1-\delta_2$ & &  $\delta_{3}^{\rm G} = 3\delta_3+\delta_1-\delta_2$ &\\
\hline
\multirow{2}{*}{$4mm$}& $\delta_{1}^{\rm G} = 4\delta_1 -\delta_2$ & $ \delta_{1}^{\rm G} = 4\delta_1 - \delta_2$ &  $\delta_{1}^{\rm G} = 2\delta_1$ & $\delta_{1}^{\rm G} = 2\delta_1$\\
& $\delta_{2}^{\rm G} = 2\delta_2$ & $ \delta_{2}^{\rm G} =2\delta_2$ &  & $\delta_{2}^{\rm G} = 0\mod2$\\
\hline
\multirow{2}{*}{$3$}& $\delta_{1}^{\rm G} = 3\delta_1$ & $\delta_{1}^{\rm G} = 3\delta_1$ & $\delta_{1}^{\rm G} = 3\delta_1$ & $\delta_{1}^{\rm G} = 3\delta_1$ \\
& $\delta_{2}^{\rm G} = 3\delta_2$&& $\delta_{2}^{\rm G} = 3\delta_2$&\\
\hline
\multirow{1}{*}{$3m$}& $\delta_{1}^{\rm G} = 3\delta_1$ & $\delta_{1}^{\rm G} = 3\delta_1$ & $\delta_{1}^{\rm G} = 3\delta_1$ & $\delta_{1}^{\rm G} = 3\delta_1$\\
\hline
\multirow{5}{*}{$6$}& $\delta_{1}^{\rm G} = 3\delta_1 + \delta_5 - \delta_2$ & $\delta_{1}^{\rm G} = 4\delta_1 - \delta_2$ &  $\delta_{1}^{\rm G} = 3\delta_1 + \delta_5 - \delta_2$ & $\delta_{1}^{\rm G} = 3\delta_1 - \delta_2$\\
& $\delta_{2}^{\rm G} = 2\delta_2 + \delta_5 - \delta_3$ & $\delta_{2}^{\rm G} = 2\delta_2 + \delta_1 - \delta_3$ & $\delta_{2}^{\rm G} = 2\delta_2 + \delta_5 - \delta_3$ & $\delta_{2}^{\rm G} = \delta_2$ \\
& $\delta_{3}^{\rm G} = 2\delta_3 + \delta_1 +\delta_5 - \delta_2 - \delta_4$ & $\delta_{3}^{\rm G} = 2\delta_3 + 2\delta_1 - 2\delta_2$ & $\delta_{3}^{\rm G} = 2\delta_3 + \delta_1 +\delta_5 - \delta_2 - \delta_4$ & $\delta_{3}^{\rm G} = 0\mod2$\\
& $\delta_{4}^{\rm G} = 2\delta_4 + \delta_1 - \delta_3$ && $\delta_{4}^{\rm G} = 2\delta_4 + \delta_1 - \delta_3$ &\\
& $\delta_{5}^{\rm G} = 3\delta_5 + \delta_1 - \delta_4$ && $\delta_{5}^{\rm G} = 3\delta_5 + \delta_1 - \delta_4$ &\\
\hline
\multirow{3}{*}{$6mm$}& $\delta_{1}^{\rm G} = 4\delta_1 - \delta_2$ &  $\delta_{1}^{\rm G} = 4\delta_1 - \delta_2$ & $\delta_{1}^{\rm G} = 3\delta_1 - \delta_2$ & $\delta_{1}^{\rm G} = 3\delta_1 - \delta_2$ \\
& $\delta_{2}^{\rm G} = 2\delta_2 +\delta_1 - \delta_3$ & $\delta_{2}^{\rm G} = 2\delta_2 +\delta_1 - \delta_3$ & $\delta_{2}^{\rm G} = \delta_2$ & $\delta_{2}^{\rm G} = \delta_2$ \\
& $\delta_{3}^{\rm G} = 2\delta_3 + 2\delta_1 - 2\delta_2$ & $\delta_{3}^{\rm G} = 2\delta_3 + 2\delta_1 - 2\delta_2$ &&  $\delta_{3}^{\rm G} = 0\mod2$\\
\hline
\end{tabular}

